A Real2Sim2Real Method for Robust Object Grasping with Neural Surface Reconstruction

Recent 3D-based manipulation methods either directly predict the grasp pose using 3D neural networks, or solve the grasp pose using similar objects retrieved from shape databases. However, the former faces generalizability challenges when testing with new robot arms or unseen objects; and the latter assumes that similar objects exist in the databases. We hypothesize that recent 3D modeling methods provides a path towards building digital replica of the evaluation scene that affords physical simulation and supports robust manipulation algorithm learning. We propose to reconstruct high-quality meshes from real-world point clouds using state-of-the-art neural surface reconstruction method (the Real2Sim step). Because most simulators take meshes for fast simulation, the reconstructed meshes enable grasp pose labels generation without human efforts. The generated labels can train grasp network that performs robustly in the real evaluation scene (the Sim2Real step). In synthetic and real experiments, we show that the Real2Sim2Real pipeline performs better than baseline grasp networks trained with a large dataset and a grasp sampling method with retrieval-based reconstruction. The benefit of the Real2Sim2Real pipeline comes from 1) decoupling scene modeling and grasp sampling into sub-problems, and 2) both sub-problems can be solved with sufficiently high quality using recent 3D learning algorithms and mesh-based physical simulation techniques.

==> problem_statement_old.tex <==

% \NA{This section should start with defining the input and desired output. The first paragraph is talking about evaluating neural networks, which is too early. What neural network? What are we evaluating? It is important to introduce the problem setting and task before discussing the approach or evaluation.}

Given depth maps and segmentation masks of the test scenes, camera poses as inputs, the reconstruction algorithm outputs object meshes and poses. The posed object meshes are used to train grasping networks. We evaluate the trained networks in the test scenes and use the grasp successes to measure the performance of the reconstruction framework. 

To evaluate the trained networks, we choose the task of grasping objects in clutter using 6-DOF grasp as this is a basic and important skill in robotic manipulation research. A test scene consists of objects on a table top next to a robot arm equipped with a parallel yaw gripper, illustrated in \autoref{fig:grasping_scene_illustration}
% \NA{It is somewhat disappointing that the introduction highlighted Real2Sim2Real as a key problem in manipulation research but here the focus is on Sim2Sim2Sim.}. 
The objects belong to four categories: bottle, bowl, can, and mug, taken from PartNet-Mobility and ShapeNetCorev2 \cite{shapenet, SAPIEN}. Each scene consists of $5$ to $10$ randomly chosen objects. To place the objects on the table, we generate random object poses ensuring that the objects are upright on the table and there are no intersecting between the objects.
%, and there are no object stacked on top of another object.
%We assume access to the ground truth mesh and pose of the table in the test scene. 

\begin{algorithm}[t]
 \hspace*{\algorithmicindent} \textbf{Input:} $p\_WOlist \in R^{n \times 3}$, $3D$ positions of $n$ object points expressed with respect to the world frame $W$\\
 \hspace*{\algorithmicindent} \textbf{Input:} Trained Convolutional ONet, represented by $f$\\
 \hspace*{\algorithmicindent} \textbf{Output:} A mesh constructed from the input point cloud $p\_WOlist$, expressed in the world frame $mesh\_W$
\begin{algorithmic}[1]
\State{Obtain the max and min bounds of the input point cloud}
\begin{align*}
bound\_max & = np.max(p\_WOlist, axis=0) \in R^3 \\ 
bound\_min & = np.min(p\_WOlist, axis=0) \in R^3
\end{align*}
\State{Compute normalization parameters}
\begin{align*}
center & = (bound\_max + bound\_min) / 2 \\
scale & = np.max(bound\_max - bound\_min)
\end{align*}
\State{Normalize point cloud and obtain mesh}
\begin{align*}
p\_WOlist\_norm & = (p\_WOlist - center) / scale \\
mesh\_O & = MISE( f (p\_WOlist\_norm) )
\end{align*}
\State{Transform mesh to world frame}
\begin{align*}
T\_WO & = \begin{bmatrix}
scale* I  & center \\
0 & 1
\end{bmatrix} \\
mesh\_W & = mesh\_O.apply\_transform(T\_WO)
\end{align*}
\caption{Obtaining reconstructed mesh from object-level point cloud}
\label{algo:obj_point_to_mesh}
\end{algorithmic}
\end{algorithm}

In each test scene, we place RGBD cameras such that they are above the table and they look at the center of the table. Given the RGB images and depth maps captured by the cameras, an algorithm should reconstruct a replica of the test scene in a separate simulation instance. We then use the reconstructions of the test scene to train grasping network, such as Contact-GraspNet \cite{cgn} or Volumetric Grasping Network \cite{vgn}. The performance of the reconstruction algorithm is then evaluated by the success rate of the trained grasping networks in the original test scene. Our evaluation metrics is different from the metrics used in previous works, which only evaluate the performance of the reconstruction algorithms on either pose estimation \cite{ucla2021} or Chamfer distance \cite{ditto2022}.

We demonstrate our results using test scenes in both simulation and real-world. In simulation, to better simulate challenges encountered in real world setting in our simulated test scenes, we use SimKinect, which is a popular noise model to benchmark SLAM systems \cite{handa:etal:2014, Barron:etal:2013A, Bohg:etal:2014} to add noise to the simulated depth map. We also use PhysX \cite{physx}, a state-of-the-art physics engine, to simulate the dynamics of the test scenes. Our simulated test scenes also allow us to compare the grasping successes to a retrieval-based reconstruction method \cite{ucla2021}. Our focus is not the proposal of novel grasping neural network architecture. Grasping is used to evaluate the feasibility of training networks using reconstructed digital replica of the test scenes. We therefore use existing grasping networks. We use $30$ simulated test scenes to obtain the average grasp success in our experiments.

